It's Not Always the Leader's Fault: How Informed Followers Can Undermine Efficient Leadership

Coordination facilitation and efficient decision-making are two essential components of successful leadership. In this paper, we take an informational approach and investigate how followers' information impacts coordination and efficient leadership in a model featuring a leader and a team of followers. We show that efficiency is achieved as the unique rationalizable outcome of the game when followers possess sufficiently imprecise information. In contrast, if followers have accurate information, the leader may fail to coordinate them toward the desired outcome or even take an inefficient action herself. We discuss the implications of the results for the role of leaders in the context of financial fragility and crises.

==> applications.tex <==
\section{Implications for Applications}
Our results have important implications for applications of the global games framework. In reality, most phenomena are dynamic in nature and for some, it can be the case that there exists a "special" player, the leader, whose actions may have payoff externalities as well as an informational role. In this case, we have identified conditions that can guarantee the uniqueness of rationalizable play, thus making easier the goal of analysts to perform comparative statics analysis. We have also illustrated the sensitivity of such predictions to the specific details of the information structures assumed. 

Consider for example a currency attack game, in which there is a large player, in the spirit of \cite{corsetti_et_al_2004}, who acts first. Assume that the large player perfectly knows the state as in our baseline model. As we have shown, uniqueness of rationalizable play is not guaranteed, unless the variance in the noise of the small players' signals is sufficiently high. If this is the case, then the qualitative predictions do not change. If, however, this is not true, then in principle, one cannot rule out non monotone equilibrium play.  \cmmt{more tuff here}


